Optimization of the Model Predictive Control Update Interval Using Reinforcement Learning

In control applications there is often a compromise that needs to be made with regards to the complexity and performance of the controller and the computational resources that are available. For instance, the typical hardware platform in embedded control applications is a microcontroller with limited memory and processing power, and for battery powered applications the control system can account for a significant portion of the energy consumption. We propose a controller architecture in which the computational cost is explicitly optimized along with the control objective. This is achieved by a three-part architecture where a high-level, computationally expensive controller generates plans, which a computationally simpler controller executes by compensating for prediction errors, while a recomputation policy decides when the plan should be recomputed. In this paper, we employ model predictive control (MPC) as the high-level plan-generating controller, a linear state feedback controller as the simpler compensating controller, and reinforcement learning (RL) to learn the recomputation policy. Simulation results for two examples showcase the architecture's ability to improve upon the MPC approach and find reasonable compromises weighing the performance on the control objective and the computational resources expended.

==> sections/related.tex <==
\section{Related Works}\label{sec:related}

The \gls*{lqr} arises as the optimal solution to the \gls*{mpc} optimization problem when the system equations are linear with no or only zero-mean Gaussian disturbance, and the cost is quadratic in the state and the inputs. Because of this clear relationship between the two, there has been several cross-applications of \gls*{mpc} and \gls*{lqr} in the literature. One of the first established stability proofs for the \gls*{mpc} framework, the dual-mode \gls*{mpc}, was designed around an \gls*{lqr} controller that would provide the terminal inputs, and the \gls*{mpc} would generate state trajectories that were required to end in an invariant set for the \gls*{lqr}. In this architecture, the \gls*{lqr} is never used in practice, and is only a theoretical tool to guarantee stability of the controller design. \citep{michalska_robust_1993,chen_quasi-infinite_1998}  More MPC + LQR crossovers (?)
 
As the substantial online computation cost is a major drawback of the \gls*{mpc} framework, there have been several proposed approaches to lessen this problem. Some approaches look at adjusting the sampling time to weigh the relationship between performance, stability and computation, either by having the sampling time as a decision variable of the optimization problem or as part of the cost function.\citep{hoffmann_variable_2012,cao_variable_2014,altin_model_2018}. Move blocking is a technique in which the inputs or other optimization variables are fixed to be constant over several contiguous time steps, in order to reduce the amount of decision variables in the optimization problem \citep{cagienard_move_2004}.

Even more closely linked with this work are the works that suggest combining \gls*{mpc} with other controllers to reduce the computational burden. In \cite{song_hybrid_2012} a global nonlinear controller is approximated by a number of piecewise affine linear controllers that are scheduled by a global \gls*{mpc} controller. \cite{akesson_neural_2006} train a \gls*{nn} to mimic the outputs of a \gls*{mpcr} with the intention of the \gls*{nn} controller replacing the \gls*{mpc} in online operation to reduce computational requirements. In this approach, the \gls*{mpc} is evaluated offline on systems to generate the training data for  the \gls*{nn} controller. As \gls*{nmpc} is significantly more computationally demanding than linear \gls*{mpc}, \cite{zhu_hybrid_1999} suggest decomposing the plant into nonlinear and linear subsystems and employ linear \gls*{mpc} wherever possible. They show that such an approach can reduce the computational time by an order of magnitude.
